Specular-to-Diffuse Translation for Multi-View Reconstruction

Most multi-view 3D reconstruction algorithms, especially when shape-from-shading cues are used, assume that object appearance is predominantly diffuse. To alleviate this restriction, we introduce S2Dnet, a generative adversarial network for transferring multiple views of objects with specular reflection into diffuse ones, so that multi-view reconstruction methods can be applied more effectively. Our network extends unsupervised image-to-image translation to multi-view "specular to diffuse" translation. To preserve object appearance across multiple views, we introduce a Multi-View Coherence loss (MVC) that evaluates the similarity and faithfulness of local patches after the view-transformation. Our MVC loss ensures that the similarity of local correspondences among multi-view images is preserved under the image-to-image translation. As a result, our network yields significantly better results than several single-view baseline techniques. In addition, we carefully design and generate a large synthetic training data set using physically-based rendering. During testing, our network takes only the raw glossy images as input, without extra information such as segmentation masks or lighting estimation. Results demonstrate that multi-view reconstruction can be significantly improved using the images filtered by our network. We also show promising performance on real world training and testing data.

==> training.tex <==
\section{Training Setup}


				
\begin{figure*}[t!]

\centering
	{\includegraphics[width=.49\linewidth]{figures/sift/sift1}}
	{\includegraphics[width=.49\linewidth]{figures/sift/sift2}}

	\caption{Two examples of the SIFT correspondences pre-computed for our training.}
	
\label{sift}

\end{figure*}


\subsection{Training Data}

The possibility of applying GANs in material transfer tasks has been shown in DualGAN \cite{yi2017dualgan}. However, the MATERIAL dataset used in DualGAN is relatively small and does not contain multi-view data. Therefore, as one of our main contributions, we systematically design and build a large dataset for our task. As it is impractical to capture enough real world data, we use a physically based renderer PBRT (cite) to generate training data and strive to make the training data as close to the real world data as possible.  

We have experimented with a large variation of rendering parameters and found that the combination of rendering parameters has a big impact on the performance of image-to-image translation. We have tried simpler versions of the task in the sense that the two domains of the glossy-diffuse images are more close-by. For both glossy and diffuse images, we tried applying the same metal material but with different roughness values, using the same object color for the diffuse image, or putting an infinite ground floor under the object for background simplification. While these choices of rendering parameters usually lead to better translation quality for synthetic data, they fail to generalize to real world data. On the other hand, if the translation task is too difficult, e.g., the models do not have enough geometric detail or the range of brightness and contrast is too wide, the network would under fit the data. We would also like to maximize the benefit our diffuse images bring to the stereo reconstruction pipeline while not using too much rendering budget for each image.     

We have rendered over 2 million images for trying out different versions of our training data using random rendering parameters. For the final version, after ignoring images with weak correspondence, our dataset contains 647312 images of resolution 512x512. For testing, we render additional 1000 sequences of images and each sequence contains 50 pairs of glossy-diffuse images. All the synthetic results shown in the paper are the output of test data. Below are some more details about the generation of our training data:
 
\begin{itemize}
  \item Geometry. We have collected and aligned 91 watertight and noise-free models with rich geometric details. Three of them are exclusively used in testing data. The models we selected are watertight, noise-free and most of the them are downloaded from Sketchfab \cite{sketchfab}. 
	\item Illumination. For global lighting, 20 different indoor environment map are randomly picked and positioned. A directional light that approximately pointing from the camera to the center of the object is also used, in addition to two lamp lights positioned on top of the object. The intensity and position of these lights are random.  
	\item Material. For glossy material, the metal material defined in PBRT in used, including copper, silver and gold. We also add some randomness in the roughness and color of the material. 
	\item Camera positions. We have uniformly sampled 700 ordered camera positions on the upper half surrounding sphere that viewing towards the center of model. Each time we randomly choose 5 consecutive camera positions and render 5 pairs of images while other scene parameters are the same. The camera positions are consecutive in the sense they are close to each other in clock-wise order, mimicking the general way of taking photos for stereo reconstruction. For each 5 image pairs, we obtain 3 image triplet as the input of the network.
	\item Image resolution. The size of a single image is 512x512, which makes the input of our multi-view network 1536x512. Using a larger image size would certainly lead to better 3D reconstruction, which however, would exceed our GPU memory budget. 
	\item SIFT correspondence. For each three consecutive images, we first extract feature points on all the images based on the SIFT descriptor. Then for each feature point of the middle image, we compute the corresponding feature point on the other two images with maximal SIFT similarity. We ignore those feature triplet points with too large distance in the SIFT or image space. The image triplet is ignore if the number of extracted feature triplets is smaller than 10, as we would like the network focus on the local patches with strong SIFT correspondence. In the end, each image triplet contains around 10 to 200 feature point triplets, and we use the feature point position as the center of the image patches unless the feature points locates too close to the image boundary. While training, the network randomly pick one of the computed feature triplets for the correspondence loss.
\end{itemize}




\subsection{Network Details}

Our network is built on the Pytorch implementation of cycle-GAN. We have explored a few choices of the encoder of generator, including U-Net \cite{ronneberger2015u}, ResNet \cite{}, RNN-block \cite{}. We have found that all these networks lead to similar results given enough training time. In the end, we selected U-Net as it is more memory efficient and generally converges faster than the alternatives. 
As shown in Figure~\ref{fig:network}, we use a multi-scale discriminator introduced in pin2pixHD paper with downsample rate of 2 that generally works better for high resolution images. Followed by the training guidances proposed in the Progressive-GAN paper, we use pixel-wise normalization and add a stride 1 convolutional layer after each deconvolutional layers. For the size of the corresponding patches, we have tried both 128x128 and 256x156 and in general the later yields results with higher stability. The discriminator architecture is:
C64-C128-C256-C512-C1. The generator decoder architecture is: C64-C128-C256-C512-C512-C512-C512-C512. We use $\lambda_{adv} = 10, \lambda_{cyc} = 10, \lambda_{corr} = 5$ for our loss weights. We use ADAM with learning rate of 0.0002.

\label{sec:training}


